Dynamical Audio-Visual Navigation: Catching Unheard Moving Sound Sources in Unmapped 3D Environments

Recent work on audio-visual navigation targets a single static sound in noise-free audio environments and struggles to generalize to unheard sounds. We introduce the novel dynamic audio-visual navigation benchmark in which an embodied AI agent must catch a moving sound source in an unmapped environment in the presence of distractors and noisy sounds. We propose an end-to-end reinforcement learning approach that relies on a multi-modal architecture that fuses the spatial audio-visual information from a binaural audio signal and spatial occupancy maps to encode the features needed to learn a robust navigation policy for our new complex task settings. We demonstrate that our approach outperforms the current state-of-the-art with better generalization to unheard sounds and better robustness to noisy scenarios on the two challenging 3D scanned real-world datasets Replica and Matterport3D, for the static and dynamic audio-visual navigation benchmarks. Our novel benchmark will be made available at http://dav-nav.cs.uni-freiburg.de.

==> chapters/7-summary.tex <==
\chapter{Summary of Results}
\label{chap:summary}
Integrating the proposed audio complex scenarios\ref{sec:complex} and the spectrogram reconstruction\ref{sec:aux} as an auxiliary task with the AV-WaN architecture has secured the first place in the SoundSpaces Challenge at The Conference on Computer Vision and Pattern Recognition (CVPR) 2021. This challenge was tackling the problem of generalizing to unheard sounds in Matterport3D \ref{fig:matterport3d} on the static AudioGoal setup \ref{soundspaces}. This approach outperfomed the AV-WaN baseline by 11\% points in terms of SPL metric and 21\% points on the success rate metric on the standard test dataset while on the unpublished challenge set dataset, this model increased the SPL by 13\% points and the success rate by 18\% points.

On the evaluation of static AudioGoal task without complex scenarios, the new proposed architecture alone without integrating the complex scenarios has improved the success rate by 12.5 \% points on Replica\cite{straub2019replica} and  4\% points on MP3D on the clean unheard audio setup. While by integrating the audio complex scenarios, the proposed model has increased the SPL by 26.7 \% points on Replica and 15.4 on MP3D which outperfoms the challenge's winning model as well.

While on the evaluation of static AudioGoal task with complex scenarios, the model achieved a better SPL on the unheard sounds setup by 4\% points on Replica and 6.5\% points on MP3D. The complex audio scenarios have been added to the baselines as well to ensure a fair comparison.

On the evaluation of the novel dynamic AudioGoal task without complex scenarios, the proposed mdoel alone without integrating the complex scenarios achieved a sucuess rate on the heard setup of 93.1\% on Replica and 95\% on MP3D. After adding the complex scenarios, the proposed architecture improved the success rate on the unheard sounds setup with 16.4\% points on Replica and 12.5\% points on MP3D.

While on the evaluation of dynamic AudioGoal task in presence of complex scenarios, the proposed approach outperforms the baseline on MP3D with 13.2\% points on the unheard sounds setup. The complex audio scenarios have been also added to the baselines to ensure a fair comparison.

After reviewing the previous results and the results on the Experiment chapter \ref{chap:experiments}, it is obvious that 1. The novel dynamic audio visual navigation task and the complex audio scenarios increase the complexity of the current task and cover a much broader range of scenarios. 2. Training in the presence of complex audio scenarios is beneficial for generalizing to unheard sounds and performing in a noisy environments. 3. The proposed model performs better on both tasks in clean and noisy environments.
\begin{figure}[htpb]
  \centering
    \includegraphics[width=0.9\textwidth,height=0.9\textheight, keepaspectratio]{img/examples_large.png}
    \caption{.}
    \label{fig:examples}
\end{figure}

==> tables/all.tex <==
\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
    Model & \multicolumn{6}{c|}{Replica} & \multicolumn{6}{c}{MP3D} \\
    \cmidrule{2-13}
    & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c|}{Unheard} & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c}{Unheard} \\
    \cmidrule{2-13}
    & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    % AV-Nav \cite{chen2020soundspaces} & 64.5 & -- & -- & 45.4 & -- & -- & 44.8 & -- & -- & 33.8 & -- & -- \\
    % AV-Nav \cite{chen2020learning} & -- & -- & -- & 34.7 & 50.9 & 16.7 & -- & -- & -- & 25.9 & 40.1 & 12.8 \\
    AV-Nav (reprod) & 61.3 & 80.1 & n.a & 34.1 & 51.1 & 16.7 & \textbf{53.7} & 69.8 & 30.2 & 28.3 & 38.2 & 14.8 \\ 
    % AV-WaN \cite{chen2020learning} & -- & -- & -- & 34.7 & 52.8 & 27.1 & -- & -- & -- & 40.9 & 56.7 & 30.6\\
    AV-WaN (reprod) &64.5   & \textbf{91.2} & 49.1 & 27.3 & 42.5 & 20.4 & 55.4 & 81.4 & 44.0 & 39.6 & 56.6 & 31.1 \\
    new arch & \textbf{71.9}& 85.9&\textbf{53.7} & 48.6 & 63.6 & 35.4 & 66.2& \textbf{86.7}& 48.5& 46.3& 60.6& 33.8\\
    % + specto aux & 62.8 & 85.4 & 45.6 & \textbf{59.2} & \textbf{85.2} & 42.9 & 63.5& 83.3&48 &47.8 &58.4 &34.15 \\
    % + dynamic &  &  &  & & & & 49.8&73 & 34.6&35.7 &48.6 &24.8 \\
    \midrule
    AV-Nav + complex &63.3 &86.1 &32.2 & 44.3&63.4& 21.3&50.7 &70.3 &29.7 & 32.6 &48.8&17.2\\
    AV-WaN + complex & 62.9&86.4 &48.2 & 47.8& 73.7&36.2 &59.6 &\textbf{86.}7 &45.5 & 47.4&69.4 &35.6 \\
    % + complex &  &  &  &  & & &59.8 &79.7 & 44.4 & 46.4 & 66.0 & 34.3  \\ 
    new + complex - aux & 51.2 & 75.6 & 35.2 & \textbf{54(53.2)} & \textbf{78(79.4)} &\textbf{(36.7)} & \textbf{66.3}& 86.4& \textbf{47.7}& \textbf{55 (54.2)} & \textbf{73(75.6)} & \textbf{(38.6)}  \\ 
    new + complex - aux + dynamic & \textcolor{blue}{46.9} & \textcolor{blue}{60.8} & \textcolor{blue}{34.8} & \textcolor{blue}{37.4}&\textcolor{blue}{52.7} &\textcolor{blue}{27.5} & \textbf{66.4}& 84.1& \textbf{48.9}& 48.6& 65.3&35.6 \\
    %  + complex + aux(0.005) &  &  &  &  &  & & 60.9& 80&45.9 & 54.9 &74.3 & \textbf{40.6}  \\ 
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{without} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments }
  \label{tab:static}
\end{table*}


\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
    Model & \multicolumn{6}{c|}{Replica} & \multicolumn{6}{c}{MP3D} \\
    \cmidrule{2-13}
    & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c|}{Unheard} & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c}{Unheard} \\
    \cmidrule{2-13}
    & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    AV-Nav + complex &55.3 &\textbf{81.1} &27.5 & 43.8 & 65.1 & 21.5& 46.7& 69.4& 25.6&36.9&56.1&19.4\\
    AV-WaN + complex  &\textbf{54.0} &80.0 &\textbf{40.9} & 43.0& 66.5&32.3 & 57.6& \textbf{84.6} & \textbf{45.6}&49.0 & 72.3 & 37.3  \\
    % + complex &  &  &  &  & & &55.6 &76.9 & 41.5& 47.8 & 68.0 & 35.6  \\ 
    new + complex - aux & 47.9 & 73.7 & 33.1 &  \textbf{47.8}& \textbf{73.4}& \textbf{33.3}& \textbf{60.5}& 84.4& 43.0& \textbf{54.5} & \textbf{75.1} & \textbf{39.1} \\ 
     
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{with} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments }
  \label{tab:static_complex}
\end{table*}


\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{l|ccc|ccc|ccc|ccc}
    \toprule
    Model & \multicolumn{6}{c|}{Replica} & \multicolumn{6}{c}{MP3D} \\
    \cmidrule{2-13}
    & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c|}{Unheard} & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c}{Unheard} \\
    \cmidrule{2-13}
    & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA \\
    \midrule
    AV-Nav & 44.0 &  69.5 & 14.6 & 22.3 & 35.0 & 7.5  & 39.9 & 70.1 & 16.4 & 21.8 & 38.7 & 8.8 \\ 
    AV-WaN &  56.6& 88.8 & 33.3 & 23.9 & 38.7 & 13.9 & 57.9 & 85.8 & 34.9 &  26.2 & 38.4 & 16.0 \\
    new arch & \textbf{62.4} & \textbf{93.1} & 33.6 & 23.1 & 36.0 & 12.4 & \textbf{63.9} & \textbf{95.0} & \textbf{36.7} & 29.9   & 46.3 & 17.6\\
    % +aux & 58 & 89.4 &  &  28&  45.5&  & 51.9 &88.3  &  &  38.9 & 63.4 &\\
    \midrule
    % + complex scenarios &  &  &  & 25.1 & 55.2 &  &  &  &  &  &  &   \\ 
    AV-Nav + complex& 43.1& 67.0& 14.6& 23.5& 38.4&7.5&37.7&67.3&15.5&20.4&35.5&8.4 \\
    AV-WaN + complex & 47.3 & 75.0 & 28.3&29.4&51.6 & \textbf{17.6}& 55.4& 86.7& 33.8 &36.2 &61.5 & 22.1\\
    new + complex scenarios - aux & 36.2 & 57.7 & 20.7 & \textbf{29.9} & \textbf{68(58.6)} & 17.0 &  61.6 &  91.9 & 36.2 & \textbf{45.8} & \textbf{74(73.4)} & \textbf{26.0}  \\ 
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{dynamic} Audio Goal task \textbf{without} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments}
  \label{tab:dynamic}
\end{table*}


\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c|}{Replica} & \multicolumn{6}{c}{MP3D} \\
    \cmidrule{2-13}
    & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c|}{Unheard} & \multicolumn{3}{c|}{Multiple Heard} & \multicolumn{3}{c}{Unheard} \\
    \cmidrule{2-13}
    Model & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA \\
    \midrule
    AV-Nav + complex & 32.9&60.1&10.5 & 25.5& 45.2 &8.1 & 35.6 & 62.6 & 13.7 & 25.1 & 44.3 &9.7\\ 
    AV-WaN + complex & \textbf{44}&\textbf{66.1} &\textbf{25.6} & \textbf{34.2}&52.1 &\textbf{19.9} & 53.7 & 84.6 & 32.9 & 42.9 & 70.9 & 26.2\\
    new arch + complex - aux & 32.6 & 55.3 & 18.8 & 27.5 &\textbf{52.6}  &16.1  & \textbf{59.9(59)(57.8)} & \textbf{92.8(91.5) (93.2)} & \textbf{33.3} & \textbf{49.2(49.5)(52.1)} & \textbf{80.5(80.9)(84.1)}& 30.4  \\ 
     
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{dynamic} Audio Goal task \textbf{with} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments}
  \label{tab:dynamic_complex}
\end{table*}

\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{\textit{Replica}} & \multicolumn{6}{c}{\textit{MP3D}} \\
    & \multicolumn{3}{c}{\textit{Multiple Heard}} & \multicolumn{3}{c}{\textit{Unheard}} & \multicolumn{3}{c}{\textit{Multiple Heard}} & \multicolumn{3}{c}{\textit{Unheard}} \\
    Model & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    AV-Nav \cite{chen2020soundspaces} & 64.5 & -- & -- & 45.4 & -- & -- & 44.8 & -- & -- & 33.8 & -- & -- \\
    AV-Nav \cite{chen2020learning} & -- & -- & -- & 34.7 & 50.9 & 16.7 & -- & -- & -- & 25.9 & 40.1 & 12.8 \\
    AV-Nav (reprod) & 61.3 & 80.1 & n.a & 34.1 & 51.1 & 16.7 & \textbf{53.7} & 69.8 & 30.2 & 28.3 & 38.2 & 14.8 \\ 
    AV-WaN \cite{chen2020learning} & -- & -- & -- & 34.7 & 52.8 & 27.1 & -- & -- & -- & 40.9 & 56.7 & 30.6\\
    AV-WaN (reprod) &64.5   & \textbf{91.2} & \textbf{49.1} & 27.3 & 42.5 & 20.4 &  &  &  & 40.9 & 56.7 & 30.6 \\
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{without} complex scenarios. Reproduction of the baselines.}
  \label{tab:reprod}
\end{table*}


\begin{table}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc@{}}
    \toprule
   Model & \multicolumn{6}{c}{Replica} \\
    & & Heard & & & Unheard \\
     & SPL & SR & SNA & SPL & SR & SNA   \\
    \midrule
    Default & 62.8 & 85.4 & 45.6 & \textbf{59.2} & \textbf{85.2} & 42.9 \\
    + augment & &  &  & 56.1 & 82.7 & 40 \\
    + secondAudio & &  & &  58.2 & 82.7 & 41.9  \\
    + specaugment + secondAudio & &  & &  57.4 & 85.2 & 40.9  \\
    + distractor & \\
    + train with moving & \\
    
     
    \bottomrule
  \end{tabular}
  \caption{}
  \label{tab:complex}
\end{table}









\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{$Replica$} & \multicolumn{6}{c}{$MP3D$} \\
    & & $Heard$ & & & $Unheard$ &  & & $Heard$ & & & $Unheard$ &  \\
    Model & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    AV-Nav + complex &55.3 &\textbf{81.1} &27.5 & 43.8 & 65.1 & 21.5& 46.7& 69.4& 25.6&36.9&56.1&19.4\\
    AV-WaN + complex  &\textbf{54} &80 &\textbf{40.9} & 43& 66.5&32.3 & 57.6& \textbf{84.6} & \textbf{45.6}&49 & 72.3 & 37.3  \\
    % + complex &  &  &  &  & & &55.6 &76.9 & 41.5& 47.8 & 68.0 & 35.6  \\ 
    new + complex - aux & 47.9 & 73.7 & 33.1 &  \textbf{47.8}& \textbf{73.4}& \textbf{33.3}& \textbf{60.5}& 84.4& 43& \textbf{54.5} & \textbf{75.1} & \textbf{39.1} \\ 
     
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{with} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments }
  \label{tab:static_complex}
\end{table*}


\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{$Replica$} & \multicolumn{6}{c}{$MP3D$} \\
    & & $Heard$ & & & $Unheard$ &  & & $Heard$ & & & $Unheard$ &  \\
    Model & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA \\
    \midrule
    AV-Nav + complex & 32.9&60.1&10.5 & 25.5& 45.2 &8.1 & 35.6 & 62.6 & 13.7 & 25.1 & 44.3 &9.7\\ 
    AV-WaN + complex & \textbf{44}&\textbf{66.1} &\textbf{25.6} & \textbf{34.2}&52.1 &\textbf{19.9} & 53.7 & 84.6 & 32.9 & 42.9 & 70.9 & 26.2\\
    new arch + complex scenarios - aux & 32.6 & 55.3 & 18.8 & 27.5 &\textbf{52.6}  &16.1  & \textbf{59.9(59)(57.8)} & \textbf{92.8(91.5) (93.2)} & \textbf{33.3} & \textbf{49.2(49.5)(52.1)} & \textbf{80.5(80.9)(84.1)}& 30.4  \\ 
     
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{Active Audio Tracking} task \textbf{with} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments}
  \label{tab:dynamic_complex}
\end{table*}


\begin{table}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{$Replica$} \\
    & & $Heard$ & & & $Unheard$ \\
    Model & SPL & SR & SNA & SPL & SR & SNA   \\
    \midrule
    Default & 62.8 & 85.4 & 45.6 & \textbf{59.2} & \textbf{85.2} & 42.9 \\
    + augment & &  &  & 56.1 & 82.7 & 40 \\
    + secondAudio & &  & &  58.2 & 82.7 & 41.9  \\
    + specaugment + secondAudio & &  & &  57.4 & 85.2 & 40.9  \\
    + distractor & \\
    + train with moving & \\
    
     
    \bottomrule
  \end{tabular}
  \caption{}
  \label{tab:complex}
\end{table}








\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{$Replica$} & \multicolumn{6}{c}{$MP3D$} \\
    & & $Heard$ & & & $Unheard$ &  & & $Heard$ & & & $Unheard$ &  \\
    Model & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    AV-Nav \cite{chen2020soundspaces} & 64.5 & -- & -- & 45.4 & -- & -- & 44.8 & -- & -- & 33.8 & -- & -- \\
    AV-Nav \cite{chen2020learning} & -- & -- & -- & 34.7 & 50.9 & 16.7 & -- & -- & -- & 25.9 & 40.1 & 12.8 \\
    AV-Nav (reprod) & 61.3 & 80.1 & n.a & 34.1 & 51.1 & 16.7 & \textbf{53.7} & 69.8 & 30.2 & 28.3 & 38.2 & 14.8 \\ 
    AV-WaN \cite{chen2020learning} & -- & -- & -- & 34.7 & 52.8 & 27.1 & -- & -- & -- & 40.9 & 56.7 & 30.6\\
    AV-WaN (reprod) &64.5   & \textbf{91.2} & \textbf{49.1} & 27.3 & 42.5 & 20.4 &  &  &  & 40.9 & 56.7 & 30.6 \\
    new arch & \textbf{71.9}& 85.9&53.7 & 48.6 & 63.6 & 35.4 & 66.2& \textbf{86.7}& 48.5& 46.3& 60.6& 33.8\\
    % + specto aux & 62.8 & 85.4 & 45.6 & \textbf{59.2} & \textbf{85.2} & 42.9 & 63.5& 83.3&48 &47.8 &58.4 &34.15 \\
    % + dynamic &  &  &  & & & & 49.8&73 & 34.6&35.7 &48.6 &24.8 \\
    \midrule
    AV-Nav + complex &64.4 &88.4 & & 44.3&63.4& &50.7 &70.3 &29.7 & 32.6 &48.8&17.2\\
    AV-WaN + complex & 62.9&86.4 &48.2 & 47.8& 73.7&36.2 &59.6 &\textbf{86.}7 &45.5 & 47.4&69.4 &35.6 \\
    % + complex &  &  &  &  & & &59.8 &79.7 & 44.4 & 46.4 & 66.0 & 34.3  \\ 
    new + complex - aux & 51.2 & 75.6 & 35.2 & \textbf{54(53.2)} & \textbf{78(79.4)} &\textbf{(36.7)} & \textbf{66.3}& 86.4& \textbf{47.7}& \textbf{55 (54.2)} & \textbf{73(75.6)} & \textbf{(38.6)}  \\ 
    new + complex - aux + dynamic &  &  &  & & & & \textbf{66.4}& 84.1& \textbf{48.9}& 48.6& 65.3&35.6 \\
    %  + complex + aux(0.005) &  &  &  &  &  & & 60.9& 80&45.9 & 54.9 &74.3 & \textbf{40.6}  \\ 
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{without} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments }
  \label{tab:static}
\end{table*}


\begin{table*}
  \footnotesize
  \centering
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{$Replica$} & \multicolumn{6}{c}{$MP3D$} \\
    & & $Heard$ & & & $Unheard$ &  & & $Heard$ & & & $Unheard$ &  \\
    Model & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA  & DSPL & SR & SNA \\
    \midrule
    AV-Nav & 44 &  69.5 & 14.6 & 22.3 & 35 & 7.5  & 39.9 & 70.1 & 16.4 & 21.8 & 38.7 & 8.8 \\ 
    AV-WaN &  56.6& 88.8 & 33.3 & 23.9 & 38.7 & 13.9 & 57.9 & 85.8 & 34.9 &  26.2 & 38.4 & 16 \\
    new arch & \textbf{62.4} & \textbf{93.1} & 33.6 & 23.1 & 36 & 12.4 & \textbf{63.9} & \textbf{95} & \textbf{36.7} & 29.9   & 46.3 & 17.6\\
    +aux & 58 & 89.4 &  &  28&  45.5&  & 51.9 &88.3  &  &  38.9 & 63.4 &\\
    \midrule
    % + complex scenarios &  &  &  & 25.1 & 55.2 &  &  &  &  &  &  &   \\ 
    AV-Nav + complex& 43.1& 67& 14.6& 23.5& 38.4&7.5&37.7&67.3&15.5&20.4&35.5&8.4 \\
    AV-WaN + complex & 47.3 & 75 & 28.3&29.4&51.6 & \textbf{17.6}& 55.4& 86.7& 33.8 &36.2 &61.5 & 22.1\\
    new + complex scenarios - aux & 36.2 & 57.7 & 20.7 & \textbf{29.9} & \textbf{68(58.6)} & 17 &  61.6 &  91.9 & 36.2 & \textbf{45.8} & \textbf{74(73.4)} & \textbf{26}  \\ 
     
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{Active Audio Tracking} task \textbf{without} complex scenarios. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments while the unheard sounds experiments represent experiments trained on multiple sounds and evaluated on unheard multiple sounds in unseen environments}
  \label{tab:dynamic}
\end{table*}




%\begin{table*}
%  \centering
%  \begin{tabular}{@{}lcccc|cccc@{}}
%    \toprule
%    Dataset & \multicolumn{4}{c}{Replica} & \multicolumn{4}{c}{MP3D} \\
%    Model & heard & unheard & moving heard & moving unheard & heard & unheard & moving %heard & moving unheard \\
%    \midrule
%    av-nav & 76 & 45 & n.a & n.a & 55 & 34 & n.a & n.a\\ 
%    waypoints & 86.6 & 34.7 & n.a & n.a & 72.3 & 40.1 & n.a & n.a\\
%    new arch \\
%    + challenge &  & 54 & n.a & n.a &  & 55 & n.a & n.a \\  
%    \bottomrule
%  \end{tabular}
%  \caption{SPL Results.   Ours is better.}
%  \label{tab:dynamic}
%\end{table*}


==> tables/baseline_reproduction.tex <==
\begin{table*}
  \footnotesize
  \centering
    \setlength{\tabcolsep}{2.5pt}
  \begin{tabular}{@{}l|ccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{6}{c}{\textit{Replica}} & \multicolumn{6}{c}{\textit{MP3D}} \\
    & \multicolumn{3}{c}{\textit{Multiple Heard}} & \multicolumn{3}{c}{\textit{Unheard}} & \multicolumn{3}{c}{\textit{Multiple Heard}} & \multicolumn{3}{c}{\textit{Unheard}} \\
    Model & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA  & SPL & SR & SNA \\
    \midrule
    AV-Nav \cite{chen2020soundspaces} & 64.5 & -- & -- & 45.4 & -- & -- & 44.8 & -- & -- & 33.8 & -- & -- \\
    AV-Nav \cite{chen2020learning} & -- & -- & -- & 34.7 & 50.9 & 16.7 & -- & -- & -- & 25.9 & 40.1 & 12.8 \\
    AV-Nav (reprod) & 61.3 & 80.1 & n.a & 34.1 & 51.1 & 16.7 & \textbf{53.7} & 69.8 & 30.2 & 28.3 & 38.2 & 14.8 \\ 
    AV-WaN \cite{chen2020learning} & -- & -- & -- & 34.7 & 52.8 & 27.1 & -- & -- & -- & 40.9 & 56.7 & 30.6\\
    AV-WaN (reprod) &64.5   & \textbf{91.2} & \textbf{49.1} & 27.3 & 42.5 & 20.4 &  &  &  & 40.9 & 56.7 & 30.6 \\
    \bottomrule
  \end{tabular}
  \caption{Results on \textbf{static} Audio Goal task \textbf{without} complex scenarios. Reproduction of the baselines.}
  \label{tab:reprod}
\end{table*}


==> tables/cont.tex <==
\begin{table*}
  %\footnotesize
  \centering
    \setlength{\tabcolsep}{6pt}
  \begin{tabular}{l|ccc}
    \toprule
    Model & \multicolumn{3}{c}{Replica}  \\

    & \multicolumn{3}{c}{Multiple Heard}  \\
    & SPL & SR & SNA   \\
    \midrule
    Ours & \textbf{71.9}& \textbf{85.9} &\textbf{53.7} \\
    + specto aux & 62.8 & 85.4 & 45.6  \\


    %  + complex + aux(0.005) &  &  &  &  &  & & 60.9& 80&45.9 & 54.9 &74.3 & \textbf{40.6}  \\ 
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{Comparison between the results of our model with and without spectrogram reconstruction as an auxiliary task on the \textbf{static} Audio Goal task \textbf{without} complex scenarios setup. The heard experiments represent experiments trained on multiple sounds and evaluated on the same sounds but in unseen environments. The unheard sounds experiments represent experiments trained on multiple sounds and evaluated on multiple unheard sounds in unseen environments.}
  \label{tab:cont}
  %\vspace{-0.3cm}
\end{table*}

